A Quantitative Comparison of Epistemic Uncertainty Maps Applied to Multi-Class Segmentation

Uncertainty assessment has gained rapid interest in medical image analysis. A popular technique to compute epistemic uncertainty is the Monte-Carlo (MC) dropout technique. From a network with MC dropout and a single input, multiple outputs can be sampled. Various methods can be used to obtain epistemic uncertainty maps from those multiple outputs. In the case of multi-class segmentation, the number of methods is even larger as epistemic uncertainty can be computed voxelwise per class or voxelwise per image. This paper highlights a systematic approach to define and quantitatively compare those methods in two different contexts: class-specific epistemic uncertainty maps (one value per image, voxel and class) and combined epistemic uncertainty maps (one value per image and voxel). We applied this quantitative analysis to a multi-class segmentation of the carotid artery lumen and vessel wall, on a multi-center, multi-scanner, multi-sequence dataset of (MR) images. We validated our analysis over 144 sets of hyperparameters of a model. Our main analysis considers the relationship between the order of the voxels sorted according to their epistemic uncertainty values and the misclassification of the prediction. Under this consideration, the comparison of combined uncertainty maps reveals that the multi-class entropy and the multi-class mutual information statistically out-perform the other combined uncertainty maps under study. In a class-specific scenario, the one-versus-all entropy statistically out-performs the class-wise entropy, the class-wise variance and the one versus all mutual information. The class-wise entropy statistically out-performs the other class-specific uncertainty maps in terms of calibration. We made a python package available to reproduce our analysis on different data and tasks.

==> figures/dice.tex <==
% This file was created by tikzplotlib v0.9.4.
\begin{tikzpicture}

\definecolor{color0}{rgb}{1,0.647058823529412,0}
\definecolor{color1}{rgb}{0.96078431372549,0.870588235294118,0.701960784313725}
\definecolor{color2}{rgb}{0.75,0,0.75}

\begin{groupplot}[group style={group size=3 by 1}]
\nextgroupplot[
tick align=outside,
tick pos=left,
title={Background},
x grid style={white!69.0196078431373!black},
xmin=-0.05, xmax=1.05,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ymin=0, ymax=151.2,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:3.46944695195361e-18,0) rectangle (axis cs:0.04,0);
\draw[draw=none,fill=color0] (axis cs:0.04,0) rectangle (axis cs:0.08,0);
\draw[draw=none,fill=color0] (axis cs:0.08,0) rectangle (axis cs:0.12,0);
\draw[draw=none,fill=color0] (axis cs:0.12,0) rectangle (axis cs:0.16,0);
\draw[draw=none,fill=color0] (axis cs:0.16,0) rectangle (axis cs:0.2,0);
\draw[draw=none,fill=color0] (axis cs:0.2,0) rectangle (axis cs:0.24,0);
\draw[draw=none,fill=color0] (axis cs:0.24,0) rectangle (axis cs:0.28,0);
\draw[draw=none,fill=color0] (axis cs:0.28,0) rectangle (axis cs:0.32,0);
\draw[draw=none,fill=color0] (axis cs:0.32,0) rectangle (axis cs:0.36,0);
\draw[draw=none,fill=color0] (axis cs:0.36,0) rectangle (axis cs:0.4,0);
\draw[draw=none,fill=color0] (axis cs:0.4,0) rectangle (axis cs:0.44,0);
\draw[draw=none,fill=color0] (axis cs:0.44,0) rectangle (axis cs:0.48,0);
\draw[draw=none,fill=color0] (axis cs:0.48,0) rectangle (axis cs:0.52,0);
\draw[draw=none,fill=color0] (axis cs:0.52,0) rectangle (axis cs:0.56,0);
\draw[draw=none,fill=color0] (axis cs:0.56,0) rectangle (axis cs:0.6,0);
\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:0.64,0);
\draw[draw=none,fill=color0] (axis cs:0.64,0) rectangle (axis cs:0.68,0);
\draw[draw=none,fill=color0] (axis cs:0.68,0) rectangle (axis cs:0.72,0);
\draw[draw=none,fill=color0] (axis cs:0.72,0) rectangle (axis cs:0.76,0);
\draw[draw=none,fill=color0] (axis cs:0.76,0) rectangle (axis cs:0.8,0);
\draw[draw=none,fill=color0] (axis cs:0.8,0) rectangle (axis cs:0.84,0);
\draw[draw=none,fill=color0] (axis cs:0.84,0) rectangle (axis cs:0.88,0);
\draw[draw=none,fill=color0] (axis cs:0.88,0) rectangle (axis cs:0.92,0);
\draw[draw=none,fill=color0] (axis cs:0.92,0) rectangle (axis cs:0.96,0);
\draw[draw=none,fill=color0] (axis cs:0.96,0) rectangle (axis cs:1,144);
\draw (axis cs:0.005,94.5) node[
  scale=0.75,
  fill=color1,
  draw=black,
  line width=0.4pt,
  inner sep=3pt,
  fill opacity=0.5,
  rounded corners,
  anchor=base west,
  text=black,
  rotate=0.0,
  align=left
]{$\mu = 0.987$


$\sigma = 0.005$};

\nextgroupplot[
tick align=outside,
tick pos=left,
title={Vessel Wall},
x grid style={white!69.0196078431373!black},
xmin=-0.05, xmax=1.05,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ymin=0, ymax=23.1,
ytick style={color=black}
]
\draw[draw=none,fill=green!50!black] (axis cs:3.46944695195361e-18,0) rectangle (axis cs:0.04,4);
\draw[draw=none,fill=green!50!black] (axis cs:0.04,0) rectangle (axis cs:0.08,0);
\draw[draw=none,fill=green!50!black] (axis cs:0.08,0) rectangle (axis cs:0.12,0);
\draw[draw=none,fill=green!50!black] (axis cs:0.12,0) rectangle (axis cs:0.16,0);
\draw[draw=none,fill=green!50!black] (axis cs:0.16,0) rectangle (axis cs:0.2,1);
\draw[draw=none,fill=green!50!black] (axis cs:0.2,0) rectangle (axis cs:0.24,3);
\draw[draw=none,fill=green!50!black] (axis cs:0.24,0) rectangle (axis cs:0.28,3);
\draw[draw=none,fill=green!50!black] (axis cs:0.28,0) rectangle (axis cs:0.32,1);
\draw[draw=none,fill=green!50!black] (axis cs:0.32,0) rectangle (axis cs:0.36,7);
\draw[draw=none,fill=green!50!black] (axis cs:0.36,0) rectangle (axis cs:0.4,12);
\draw[draw=none,fill=green!50!black] (axis cs:0.4,0) rectangle (axis cs:0.44,7);
\draw[draw=none,fill=green!50!black] (axis cs:0.44,0) rectangle (axis cs:0.48,4);
\draw[draw=none,fill=green!50!black] (axis cs:0.48,0) rectangle (axis cs:0.52,5);
\draw[draw=none,fill=green!50!black] (axis cs:0.52,0) rectangle (axis cs:0.56,7);
\draw[draw=none,fill=green!50!black] (axis cs:0.56,0) rectangle (axis cs:0.6,17);
\draw[draw=none,fill=green!50!black] (axis cs:0.6,0) rectangle (axis cs:0.64,19);
\draw[draw=none,fill=green!50!black] (axis cs:0.64,0) rectangle (axis cs:0.68,12);
\draw[draw=none,fill=green!50!black] (axis cs:0.68,0) rectangle (axis cs:0.72,18);
\draw[draw=none,fill=green!50!black] (axis cs:0.72,0) rectangle (axis cs:0.76,22);
\draw[draw=none,fill=green!50!black] (axis cs:0.76,0) rectangle (axis cs:0.8,2);
\draw[draw=none,fill=green!50!black] (axis cs:0.8,0) rectangle (axis cs:0.84,0);
\draw[draw=none,fill=green!50!black] (axis cs:0.84,0) rectangle (axis cs:0.88,0);
\draw[draw=none,fill=green!50!black] (axis cs:0.88,0) rectangle (axis cs:0.92,0);
\draw[draw=none,fill=green!50!black] (axis cs:0.92,0) rectangle (axis cs:0.96,0);
\draw[draw=none,fill=green!50!black] (axis cs:0.96,0) rectangle (axis cs:1,0);
\draw (axis cs:0.005,14.4375) node[
  scale=0.75,
  fill=color1,
  draw=black,
  line width=0.4pt,
  inner sep=3pt,
  fill opacity=0.5,
  rounded corners,
  anchor=base west,
  text=black,
  rotate=0.0,
  align=left
]{$\mu = 0.555$


$\sigma = 0.175$};

\nextgroupplot[
tick align=outside,
tick pos=left,
title={Lumen},
x grid style={white!69.0196078431373!black},
xmin=-0.05, xmax=1.05,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ymin=0, ymax=35.7,
ytick style={color=black}
]
\draw[draw=none,fill=color2] (axis cs:3.46944695195361e-18,0) rectangle (axis cs:0.04,5);
\draw[draw=none,fill=color2] (axis cs:0.04,0) rectangle (axis cs:0.08,0);
\draw[draw=none,fill=color2] (axis cs:0.08,0) rectangle (axis cs:0.12,0);
\draw[draw=none,fill=color2] (axis cs:0.12,0) rectangle (axis cs:0.16,0);
\draw[draw=none,fill=color2] (axis cs:0.16,0) rectangle (axis cs:0.2,0);
\draw[draw=none,fill=color2] (axis cs:0.2,0) rectangle (axis cs:0.24,0);
\draw[draw=none,fill=color2] (axis cs:0.24,0) rectangle (axis cs:0.28,0);
\draw[draw=none,fill=color2] (axis cs:0.28,0) rectangle (axis cs:0.32,0);
\draw[draw=none,fill=color2] (axis cs:0.32,0) rectangle (axis cs:0.36,0);
\draw[draw=none,fill=color2] (axis cs:0.36,0) rectangle (axis cs:0.4,0);
\draw[draw=none,fill=color2] (axis cs:0.4,0) rectangle (axis cs:0.44,0);
\draw[draw=none,fill=color2] (axis cs:0.44,0) rectangle (axis cs:0.48,0);
\draw[draw=none,fill=color2] (axis cs:0.48,0) rectangle (axis cs:0.52,5);
\draw[draw=none,fill=color2] (axis cs:0.52,0) rectangle (axis cs:0.56,7);
\draw[draw=none,fill=color2] (axis cs:0.56,0) rectangle (axis cs:0.6,6);
\draw[draw=none,fill=color2] (axis cs:0.6,0) rectangle (axis cs:0.64,13);
\draw[draw=none,fill=color2] (axis cs:0.64,0) rectangle (axis cs:0.68,12);
\draw[draw=none,fill=color2] (axis cs:0.68,0) rectangle (axis cs:0.72,8);
\draw[draw=none,fill=color2] (axis cs:0.72,0) rectangle (axis cs:0.76,13);
\draw[draw=none,fill=color2] (axis cs:0.76,0) rectangle (axis cs:0.8,20);
\draw[draw=none,fill=color2] (axis cs:0.8,0) rectangle (axis cs:0.84,19);
\draw[draw=none,fill=color2] (axis cs:0.84,0) rectangle (axis cs:0.88,34);
\draw[draw=none,fill=color2] (axis cs:0.88,0) rectangle (axis cs:0.92,2);
\draw[draw=none,fill=color2] (axis cs:0.92,0) rectangle (axis cs:0.96,0);
\draw[draw=none,fill=color2] (axis cs:0.96,0) rectangle (axis cs:1,0);
\draw (axis cs:0.005,22.3125) node[
  scale=0.75,
  fill=color1,
  draw=black,
  line width=0.4pt,
  inner sep=3pt,
  fill opacity=0.5,
  rounded corners,
  anchor=base west,
  text=black,
  rotate=0.0,
  align=left
]{$\mu = 0.718$


$\sigma = 0.174$};
\end{groupplot}

\end{tikzpicture}


==> figures/statistical_tests/AUCPRClassWiseMetric_0.tex <==
\begin{tabular}{p{0.167\textwidth}p{0.167\textwidth}p{0.167\textwidth}p{0.167\textwidth}p{0.167\textwidth}}
\hline
{} &     Class-wise \newline Variance &      One vs all \newline Entropy &           One vs all \newline MI \\
\hline
Class-wise \newline Entropy  &  $\textbf{[0.31, 0.46]}$ &   $\textbf{[0.09, 0.2]}$ &          $[0.39, 0.55]$ \\
Class-wise \newline Variance &                         &  $\textbf{[0.07, 0.17]}$ &   $\textbf{[0.9, 0.98]}$ \\
One vs all \newline Entropy  &                         &                         &  $\textbf{[0.87, 0.96]}$ \\
\hline
\end{tabular}


==> figures/statistical_tests/AUCPRClassWiseMetric_1.tex <==
\begin{tabular}{p{0.167\textwidth}p{0.167\textwidth}p{0.167\textwidth}p{0.167\textwidth}p{0.167\textwidth}}
\hline
{} &     Class-wise \newline Variance &      One vs all \newline Entropy &           One vs all \newline MI \\
\hline
Class-wise \newline Entropy  &  $\textbf{[0.26, 0.41]}$ &  $\textbf{[0.03, 0.11]}$ &          $[0.36, 0.52]$ \\
Class-wise \newline Variance &                         &  $\textbf{[0.03, 0.11]}$ &  $\textbf{[0.94, 0.99]}$ \\
One vs all \newline Entropy  &                         &                         &  $\textbf{[0.92, 0.98]}$ \\
\hline
\end{tabular}


==> figures/statistical_tests/AUCPRClassWiseMetric_2.tex <==
\begin{tabular}{p{0.167\textwidth}p{0.167\textwidth}p{0.167\textwidth}p{0.167\textwidth}p{0.167\textwidth}}
\hline
{} &     Class-wise \newline Variance &      One vs all \newline Entropy &          One vs all \newline MI \\
\hline
Class-wise \newline Entropy  &  $\textbf{[0.33, 0.48]}$ &  $\textbf{[0.06, 0.16]}$ &         $[0.45, 0.61]$ \\
Class-wise \newline Variance &                         &  $\textbf{[0.01, 0.06]}$ &  $\textbf{[0.95, 1.0]}$ \\
One vs all \newline Entropy  &                         &                         &  $\textbf{[0.95, 1.0]}$ \\
\hline
\end{tabular}


==> figures/statistical_tests/AUCPRMetric.tex <==
\begin{tabular}{p{0.125\textwidth}p{0.125\textwidth}p{0.125\textwidth}p{0.125\textwidth}p{0.125\textwidth}p{0.125\textwidth}p{0.125\textwidth}}
\hline
{} & Averaged Variance &     Multi-class Entropy &          Multi-class MI &           Similarity BC &           Similarity KL \\
\hline
Averaged Entropy    &    $[0.41, 0.57]$ &   $\textbf{[0.65, 0.8]}$ &  $\textbf{[0.55, 0.71]}$ &  $\textbf{[0.03, 0.11]}$ &   $\textbf{[0.02, 0.1]}$ \\
Averaged Variance   &                   &  $\textbf{[0.63, 0.78]}$ &   $\textbf{[0.54, 0.7]}$ &  $\textbf{[0.01, 0.07]}$ &  $\textbf{[0.02, 0.09]}$ \\
Multi-class Entropy &                   &                         &          $[0.35, 0.51]$ &  $\textbf{[0.01, 0.07]}$ &   $\textbf{[0.0, 0.05]}$ \\
Multi-class MI      &                   &                         &                         &  $\textbf{[0.03, 0.11]}$ &  $\textbf{[0.02, 0.09]}$ \\
Similarity BC       &                   &                         &                         &                         &  $\textbf{[0.21, 0.36]}$ \\
\hline
\end{tabular}


==> figures/statistical_tests/AUCROCMetric.tex <==
\begin{tabular}{p{0.25\textwidth}p{0.25\textwidth}p{0.25\textwidth}}
\hline
{} &          Multi-class MI \\
\hline
Multi-class Entropy &  $\textbf{[0.29, 0.45]}$ \\
\hline
\end{tabular}


==> figures/statistical_tests/BRATSMetric_0.tex <==
\begin{tabular}{p{0.167\textwidth}p{0.167\textwidth}p{0.167\textwidth}p{0.167\textwidth}p{0.167\textwidth}}
\hline
{} &     Class-wise \newline Variance &     One vs all \newline Entropy &          One vs all \newline MI \\
\hline
Class-wise \newline Entropy  &  $\textbf{[0.03, 0.11]}$ &  $\textbf{[0.0, 0.04]}$ &  $\textbf{[0.0, 0.04]}$ \\
Class-wise \newline Variance &                         &  $\textbf{[0.0, 0.04]}$ &  $\textbf{[0.0, 0.03]}$ \\
One vs all \newline Entropy  &                         &                        &  $\textbf{[0.96, 1.0]}$ \\
\hline
\end{tabular}


==> figures/statistical_tests/BRATSMetric_1.tex <==
\begin{tabular}{p{0.167\textwidth}p{0.167\textwidth}p{0.167\textwidth}p{0.167\textwidth}p{0.167\textwidth}}
\hline
{} &    Class-wise \newline Variance &     One vs all \newline Entropy &           One vs all \newline MI \\
\hline
Class-wise \newline Entropy  &  $\textbf{[0.1, 0.21]}$ &  $\textbf{[0.0, 0.05]}$ &  $\textbf{[0.03, 0.11]}$ \\
Class-wise \newline Variance &                        &  $\textbf{[0.0, 0.03]}$ &   $\textbf{[0.0, 0.04]}$ \\
One vs all \newline Entropy  &                        &                        &   $\textbf{[0.97, 1.0]}$ \\
\hline
\end{tabular}


==> figures/statistical_tests/BRATSMetric_2.tex <==
\begin{tabular}{p{0.167\textwidth}p{0.167\textwidth}p{0.167\textwidth}p{0.167\textwidth}p{0.167\textwidth}}
\hline
{} &     Class-wise \newline Variance &     One vs all \newline Entropy &           One vs all \newline MI \\
\hline
Class-wise \newline Entropy  &  $\textbf{[0.06, 0.16]}$ &  $\textbf{[0.0, 0.04]}$ &  $\textbf{[0.01, 0.06]}$ \\
Class-wise \newline Variance &                         &  $\textbf{[0.0, 0.03]}$ &  $\textbf{[0.01, 0.06]}$ \\
One vs all \newline Entropy  &                         &                        &   $\textbf{[0.96, 1.0]}$ \\
\hline
\end{tabular}


==> figures/vizualize.tex <==
% This file was created by tikzplotlib v0.9.4.
\begin{tikzpicture}

\begin{groupplot}[group style={group size=6 by 3}]
\nextgroupplot[
tick pos=left,
title={T1w
pre-contrast},
xmin=-0.5, xmax=127.5,
y dir=reverse,
ylabel={Dice = 0.784},
ymin=-0.5, ymax=127.5
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=127.5, ymin=127.5, ymax=-0.5] {vizualize-072.png};

\nextgroupplot[
tick pos=left,
title={Prediction},
xmin=-0.5, xmax=127.5,
y dir=reverse,
ymin=-0.5, ymax=127.5
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=127.5, ymin=127.5, ymax=-0.5] {vizualize-073.png};

\nextgroupplot[
tick pos=left,
title={Averaged
variance},
xmin=-0.5, xmax=127.5,
y dir=reverse,
ymin=-0.5, ymax=127.5
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=127.5, ymin=127.5, ymax=-0.5] {vizualize-074.png};

\nextgroupplot[
tick pos=left,
title={Averaged
entropy},
xmin=-0.5, xmax=127.5,
y dir=reverse,
ymin=-0.5, ymax=127.5
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=127.5, ymin=127.5, ymax=-0.5] {vizualize-075.png};

\nextgroupplot[
tick pos=left,
title={BC},
xmin=-0.5, xmax=127.5,
y dir=reverse,
ymin=-0.5, ymax=127.5
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=127.5, ymin=127.5, ymax=-0.5] {vizualize-076.png};

\nextgroupplot[
tick pos=left,
title={KL},
xmin=-0.5, xmax=127.5,
y dir=reverse,
ymin=-0.5, ymax=127.5
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=127.5, ymin=127.5, ymax=-0.5] {vizualize-077.png};

\nextgroupplot[
tick pos=left,
xmin=-0.5, xmax=127.5,
y dir=reverse,
ylabel={Dice = 0.861},
ymin=-0.5, ymax=127.5
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=127.5, ymin=127.5, ymax=-0.5] {vizualize-078.png};

\nextgroupplot[
tick pos=left,
xmin=-0.5, xmax=127.5,
y dir=reverse,
ymin=-0.5, ymax=127.5
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=127.5, ymin=127.5, ymax=-0.5] {vizualize-079.png};

\nextgroupplot[
tick pos=left,
xmin=-0.5, xmax=127.5,
y dir=reverse,
ymin=-0.5, ymax=127.5
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=127.5, ymin=127.5, ymax=-0.5] {vizualize-080.png};

\nextgroupplot[
tick pos=left,
xmin=-0.5, xmax=127.5,
y dir=reverse,
ymin=-0.5, ymax=127.5
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=127.5, ymin=127.5, ymax=-0.5] {vizualize-081.png};

\nextgroupplot[
tick pos=left,
xmin=-0.5, xmax=127.5,
y dir=reverse,
ymin=-0.5, ymax=127.5
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=127.5, ymin=127.5, ymax=-0.5] {vizualize-082.png};

\nextgroupplot[
tick pos=left,
xmin=-0.5, xmax=127.5,
y dir=reverse,
ymin=-0.5, ymax=127.5
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=127.5, ymin=127.5, ymax=-0.5] {vizualize-083.png};

\nextgroupplot[
tick pos=left,
xmin=-0.5, xmax=127.5,
y dir=reverse,
ylabel={Dice = 0.917},
ymin=-0.5, ymax=127.5
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=127.5, ymin=127.5, ymax=-0.5] {vizualize-084.png};

\nextgroupplot[
tick pos=left,
xmin=-0.5, xmax=127.5,
y dir=reverse,
ymin=-0.5, ymax=127.5
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=127.5, ymin=127.5, ymax=-0.5] {vizualize-085.png};

\nextgroupplot[
tick pos=left,
xmin=-0.5, xmax=127.5,
y dir=reverse,
ymin=-0.5, ymax=127.5
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=127.5, ymin=127.5, ymax=-0.5] {vizualize-086.png};

\nextgroupplot[
tick pos=left,
xmin=-0.5, xmax=127.5,
y dir=reverse,
ymin=-0.5, ymax=127.5
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=127.5, ymin=127.5, ymax=-0.5] {vizualize-087.png};

\nextgroupplot[
tick pos=left,
xmin=-0.5, xmax=127.5,
y dir=reverse,
ymin=-0.5, ymax=127.5
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=127.5, ymin=127.5, ymax=-0.5] {vizualize-088.png};

\nextgroupplot[
tick pos=left,
xmin=-0.5, xmax=127.5,
y dir=reverse,
ymin=-0.5, ymax=127.5
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=127.5, ymin=127.5, ymax=-0.5] {vizualize-089.png};
\end{groupplot}

\end{tikzpicture}


==> tables/AUCROCMetric.tex <==
\begin{tabular}{p{0.25\textwidth}p{0.25\textwidth}p{0.25\textwidth}}
\hline
{} &          Multi-class MI \\
\hline
Multi-class Entropy &  $\textbf{[0.29, 0.45]}$ \\
\hline
\end{tabular}


==> tables/ethnicity_table.tex <==
\begin{tabular}{c|c}
\hline
{} &  Ethnicity \\
\hline
Caucasian            &        141 \\
East Asia            &          2 \\
Afro-american        &          1 \\
South Asia and Hindu &          1 \\
\hline
\end{tabular}


==> tmp/figures/dice.tex <==
% This file was created by tikzplotlib v0.9.4.
\begin{tikzpicture}

\definecolor{color0}{rgb}{1,0.647058823529412,0}
\definecolor{color1}{rgb}{0.96078431372549,0.870588235294118,0.701960784313725}
\definecolor{color2}{rgb}{0.75,0,0.75}

\begin{groupplot}[group style={group size=3 by 1}]
\nextgroupplot[
tick align=outside,
tick pos=left,
title={Background},
x grid style={white!69.0196078431373!black},
xmin=-0.05, xmax=1.05,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ymin=0, ymax=151.2,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:3.46944695195361e-18,0) rectangle (axis cs:0.04,0);
\draw[draw=none,fill=color0] (axis cs:0.04,0) rectangle (axis cs:0.08,0);
\draw[draw=none,fill=color0] (axis cs:0.08,0) rectangle (axis cs:0.12,0);
\draw[draw=none,fill=color0] (axis cs:0.12,0) rectangle (axis cs:0.16,0);
\draw[draw=none,fill=color0] (axis cs:0.16,0) rectangle (axis cs:0.2,0);
\draw[draw=none,fill=color0] (axis cs:0.2,0) rectangle (axis cs:0.24,0);
\draw[draw=none,fill=color0] (axis cs:0.24,0) rectangle (axis cs:0.28,0);
\draw[draw=none,fill=color0] (axis cs:0.28,0) rectangle (axis cs:0.32,0);
\draw[draw=none,fill=color0] (axis cs:0.32,0) rectangle (axis cs:0.36,0);
\draw[draw=none,fill=color0] (axis cs:0.36,0) rectangle (axis cs:0.4,0);
\draw[draw=none,fill=color0] (axis cs:0.4,0) rectangle (axis cs:0.44,0);
\draw[draw=none,fill=color0] (axis cs:0.44,0) rectangle (axis cs:0.48,0);
\draw[draw=none,fill=color0] (axis cs:0.48,0) rectangle (axis cs:0.52,0);
\draw[draw=none,fill=color0] (axis cs:0.52,0) rectangle (axis cs:0.56,0);
\draw[draw=none,fill=color0] (axis cs:0.56,0) rectangle (axis cs:0.6,0);
\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:0.64,0);
\draw[draw=none,fill=color0] (axis cs:0.64,0) rectangle (axis cs:0.68,0);
\draw[draw=none,fill=color0] (axis cs:0.68,0) rectangle (axis cs:0.72,0);
\draw[draw=none,fill=color0] (axis cs:0.72,0) rectangle (axis cs:0.76,0);
\draw[draw=none,fill=color0] (axis cs:0.76,0) rectangle (axis cs:0.8,0);
\draw[draw=none,fill=color0] (axis cs:0.8,0) rectangle (axis cs:0.84,0);
\draw[draw=none,fill=color0] (axis cs:0.84,0) rectangle (axis cs:0.88,0);
\draw[draw=none,fill=color0] (axis cs:0.88,0) rectangle (axis cs:0.92,0);
\draw[draw=none,fill=color0] (axis cs:0.92,0) rectangle (axis cs:0.96,0);
\draw[draw=none,fill=color0] (axis cs:0.96,0) rectangle (axis cs:1,144);
\draw (axis cs:0.005,94.5) node[
  scale=0.75,
  fill=color1,
  draw=black,
  line width=0.4pt,
  inner sep=3pt,
  fill opacity=0.5,
  rounded corners,
  anchor=base west,
  text=black,
  rotate=0.0,
  align=left
]{$\mu = 0.987$


$\sigma = 0.005$};

\nextgroupplot[
tick align=outside,
tick pos=left,
title={Vessel Wall},
x grid style={white!69.0196078431373!black},
xmin=-0.05, xmax=1.05,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ymin=0, ymax=23.1,
ytick style={color=black}
]
\draw[draw=none,fill=green!50!black] (axis cs:3.46944695195361e-18,0) rectangle (axis cs:0.04,4);
\draw[draw=none,fill=green!50!black] (axis cs:0.04,0) rectangle (axis cs:0.08,0);
\draw[draw=none,fill=green!50!black] (axis cs:0.08,0) rectangle (axis cs:0.12,0);
\draw[draw=none,fill=green!50!black] (axis cs:0.12,0) rectangle (axis cs:0.16,0);
\draw[draw=none,fill=green!50!black] (axis cs:0.16,0) rectangle (axis cs:0.2,1);
\draw[draw=none,fill=green!50!black] (axis cs:0.2,0) rectangle (axis cs:0.24,3);
\draw[draw=none,fill=green!50!black] (axis cs:0.24,0) rectangle (axis cs:0.28,3);
\draw[draw=none,fill=green!50!black] (axis cs:0.28,0) rectangle (axis cs:0.32,1);
\draw[draw=none,fill=green!50!black] (axis cs:0.32,0) rectangle (axis cs:0.36,7);
\draw[draw=none,fill=green!50!black] (axis cs:0.36,0) rectangle (axis cs:0.4,12);
\draw[draw=none,fill=green!50!black] (axis cs:0.4,0) rectangle (axis cs:0.44,7);
\draw[draw=none,fill=green!50!black] (axis cs:0.44,0) rectangle (axis cs:0.48,4);
\draw[draw=none,fill=green!50!black] (axis cs:0.48,0) rectangle (axis cs:0.52,5);
\draw[draw=none,fill=green!50!black] (axis cs:0.52,0) rectangle (axis cs:0.56,7);
\draw[draw=none,fill=green!50!black] (axis cs:0.56,0) rectangle (axis cs:0.6,17);
\draw[draw=none,fill=green!50!black] (axis cs:0.6,0) rectangle (axis cs:0.64,19);
\draw[draw=none,fill=green!50!black] (axis cs:0.64,0) rectangle (axis cs:0.68,12);
\draw[draw=none,fill=green!50!black] (axis cs:0.68,0) rectangle (axis cs:0.72,18);
\draw[draw=none,fill=green!50!black] (axis cs:0.72,0) rectangle (axis cs:0.76,22);
\draw[draw=none,fill=green!50!black] (axis cs:0.76,0) rectangle (axis cs:0.8,2);
\draw[draw=none,fill=green!50!black] (axis cs:0.8,0) rectangle (axis cs:0.84,0);
\draw[draw=none,fill=green!50!black] (axis cs:0.84,0) rectangle (axis cs:0.88,0);
\draw[draw=none,fill=green!50!black] (axis cs:0.88,0) rectangle (axis cs:0.92,0);
\draw[draw=none,fill=green!50!black] (axis cs:0.92,0) rectangle (axis cs:0.96,0);
\draw[draw=none,fill=green!50!black] (axis cs:0.96,0) rectangle (axis cs:1,0);
\draw (axis cs:0.005,14.4375) node[
  scale=0.75,
  fill=color1,
  draw=black,
  line width=0.4pt,
  inner sep=3pt,
  fill opacity=0.5,
  rounded corners,
  anchor=base west,
  text=black,
  rotate=0.0,
  align=left
]{$\mu = 0.555$


$\sigma = 0.175$};

\nextgroupplot[
tick align=outside,
tick pos=left,
title={Lumen},
x grid style={white!69.0196078431373!black},
xmin=-0.05, xmax=1.05,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ymin=0, ymax=35.7,
ytick style={color=black}
]
\draw[draw=none,fill=color2] (axis cs:3.46944695195361e-18,0) rectangle (axis cs:0.04,5);
\draw[draw=none,fill=color2] (axis cs:0.04,0) rectangle (axis cs:0.08,0);
\draw[draw=none,fill=color2] (axis cs:0.08,0) rectangle (axis cs:0.12,0);
\draw[draw=none,fill=color2] (axis cs:0.12,0) rectangle (axis cs:0.16,0);
\draw[draw=none,fill=color2] (axis cs:0.16,0) rectangle (axis cs:0.2,0);
\draw[draw=none,fill=color2] (axis cs:0.2,0) rectangle (axis cs:0.24,0);
\draw[draw=none,fill=color2] (axis cs:0.24,0) rectangle (axis cs:0.28,0);
\draw[draw=none,fill=color2] (axis cs:0.28,0) rectangle (axis cs:0.32,0);
\draw[draw=none,fill=color2] (axis cs:0.32,0) rectangle (axis cs:0.36,0);
\draw[draw=none,fill=color2] (axis cs:0.36,0) rectangle (axis cs:0.4,0);
\draw[draw=none,fill=color2] (axis cs:0.4,0) rectangle (axis cs:0.44,0);
\draw[draw=none,fill=color2] (axis cs:0.44,0) rectangle (axis cs:0.48,0);
\draw[draw=none,fill=color2] (axis cs:0.48,0) rectangle (axis cs:0.52,5);
\draw[draw=none,fill=color2] (axis cs:0.52,0) rectangle (axis cs:0.56,7);
\draw[draw=none,fill=color2] (axis cs:0.56,0) rectangle (axis cs:0.6,6);
\draw[draw=none,fill=color2] (axis cs:0.6,0) rectangle (axis cs:0.64,13);
\draw[draw=none,fill=color2] (axis cs:0.64,0) rectangle (axis cs:0.68,12);
\draw[draw=none,fill=color2] (axis cs:0.68,0) rectangle (axis cs:0.72,8);
\draw[draw=none,fill=color2] (axis cs:0.72,0) rectangle (axis cs:0.76,13);
\draw[draw=none,fill=color2] (axis cs:0.76,0) rectangle (axis cs:0.8,20);
\draw[draw=none,fill=color2] (axis cs:0.8,0) rectangle (axis cs:0.84,19);
\draw[draw=none,fill=color2] (axis cs:0.84,0) rectangle (axis cs:0.88,34);
\draw[draw=none,fill=color2] (axis cs:0.88,0) rectangle (axis cs:0.92,2);
\draw[draw=none,fill=color2] (axis cs:0.92,0) rectangle (axis cs:0.96,0);
\draw[draw=none,fill=color2] (axis cs:0.96,0) rectangle (axis cs:1,0);
\draw (axis cs:0.005,22.3125) node[
  scale=0.75,
  fill=color1,
  draw=black,
  line width=0.4pt,
  inner sep=3pt,
  fill opacity=0.5,
  rounded corners,
  anchor=base west,
  text=black,
  rotate=0.0,
  align=left
]{$\mu = 0.718$


$\sigma = 0.174$};
\end{groupplot}

\end{tikzpicture}


==> tmp/figures/statistical_tests/AUCPRClassWiseMetric_0.tex <==
\begin{tabular}{p{0.167\textwidth}p{0.167\textwidth}p{0.167\textwidth}p{0.167\textwidth}p{0.167\textwidth}}
\hline
{} &     Class-wise \newline Variance &      One vs all \newline Entropy &           One vs all \newline MI \\
\hline
Class-wise \newline Entropy  &  $\textbf{[0.31, 0.46]}$ &   $\textbf{[0.09, 0.2]}$ &          $[0.39, 0.55]$ \\
Class-wise \newline Variance &                         &  $\textbf{[0.07, 0.17]}$ &   $\textbf{[0.9, 0.98]}$ \\
One vs all \newline Entropy  &                         &                         &  $\textbf{[0.87, 0.96]}$ \\
\hline
\end{tabular}


==> tmp/figures/statistical_tests/AUCPRClassWiseMetric_1.tex <==
\begin{tabular}{p{0.167\textwidth}p{0.167\textwidth}p{0.167\textwidth}p{0.167\textwidth}p{0.167\textwidth}}
\hline
{} &     Class-wise \newline Variance &      One vs all \newline Entropy &           One vs all \newline MI \\
\hline
Class-wise \newline Entropy  &  $\textbf{[0.26, 0.41]}$ &  $\textbf{[0.03, 0.11]}$ &          $[0.36, 0.52]$ \\
Class-wise \newline Variance &                         &  $\textbf{[0.03, 0.11]}$ &  $\textbf{[0.94, 0.99]}$ \\
One vs all \newline Entropy  &                         &                         &  $\textbf{[0.92, 0.98]}$ \\
\hline
\end{tabular}


==> tmp/figures/statistical_tests/AUCPRClassWiseMetric_2.tex <==
\begin{tabular}{p{0.167\textwidth}p{0.167\textwidth}p{0.167\textwidth}p{0.167\textwidth}p{0.167\textwidth}}
\hline
{} &     Class-wise \newline Variance &      One vs all \newline Entropy &          One vs all \newline MI \\
\hline
Class-wise \newline Entropy  &  $\textbf{[0.33, 0.48]}$ &  $\textbf{[0.06, 0.16]}$ &         $[0.45, 0.61]$ \\
Class-wise \newline Variance &                         &  $\textbf{[0.01, 0.06]}$ &  $\textbf{[0.95, 1.0]}$ \\
One vs all \newline Entropy  &                         &                         &  $\textbf{[0.95, 1.0]}$ \\
\hline
\end{tabular}


==> tmp/figures/statistical_tests/AUCPRMetric.tex <==
\begin{tabular}{p{0.125\textwidth}p{0.125\textwidth}p{0.125\textwidth}p{0.125\textwidth}p{0.125\textwidth}p{0.125\textwidth}p{0.125\textwidth}}
\hline
{} & Averaged Variance &     Multi-class Entropy &          Multi-class MI &           Similarity BC &           Similarity KL \\
\hline
Averaged Entropy    &    $[0.41, 0.57]$ &   $\textbf{[0.65, 0.8]}$ &  $\textbf{[0.55, 0.71]}$ &  $\textbf{[0.03, 0.11]}$ &   $\textbf{[0.02, 0.1]}$ \\
Averaged Variance   &                   &  $\textbf{[0.63, 0.78]}$ &   $\textbf{[0.54, 0.7]}$ &  $\textbf{[0.01, 0.07]}$ &  $\textbf{[0.02, 0.09]}$ \\
Multi-class Entropy &                   &                         &          $[0.35, 0.51]$ &  $\textbf{[0.01, 0.07]}$ &   $\textbf{[0.0, 0.05]}$ \\
Multi-class MI      &                   &                         &                         &  $\textbf{[0.03, 0.11]}$ &  $\textbf{[0.02, 0.09]}$ \\
Similarity BC       &                   &                         &                         &                         &  $\textbf{[0.21, 0.36]}$ \\
\hline
\end{tabular}


==> tmp/figures/statistical_tests/AUCROCMetric.tex <==
\begin{tabular}{p{0.25\textwidth}p{0.25\textwidth}p{0.25\textwidth}}
\hline
{} &          Multi-class MI \\
\hline
Multi-class Entropy &  $\textbf{[0.29, 0.45]}$ \\
\hline
\end{tabular}


==> tmp/figures/statistical_tests/BRATSMetric_0.tex <==
\begin{tabular}{p{0.167\textwidth}p{0.167\textwidth}p{0.167\textwidth}p{0.167\textwidth}p{0.167\textwidth}}
\hline
{} &     Class-wise \newline Variance &     One vs all \newline Entropy &          One vs all \newline MI \\
\hline
Class-wise \newline Entropy  &  $\textbf{[0.03, 0.11]}$ &  $\textbf{[0.0, 0.04]}$ &  $\textbf{[0.0, 0.04]}$ \\
Class-wise \newline Variance &                         &  $\textbf{[0.0, 0.04]}$ &  $\textbf{[0.0, 0.03]}$ \\
One vs all \newline Entropy  &                         &                        &  $\textbf{[0.96, 1.0]}$ \\
\hline
\end{tabular}


==> tmp/figures/statistical_tests/BRATSMetric_1.tex <==
\begin{tabular}{p{0.167\textwidth}p{0.167\textwidth}p{0.167\textwidth}p{0.167\textwidth}p{0.167\textwidth}}
\hline
{} &    Class-wise \newline Variance &     One vs all \newline Entropy &           One vs all \newline MI \\
\hline
Class-wise \newline Entropy  &  $\textbf{[0.1, 0.21]}$ &  $\textbf{[0.0, 0.05]}$ &  $\textbf{[0.03, 0.11]}$ \\
Class-wise \newline Variance &                        &  $\textbf{[0.0, 0.03]}$ &   $\textbf{[0.0, 0.04]}$ \\
One vs all \newline Entropy  &                        &                        &   $\textbf{[0.97, 1.0]}$ \\
\hline
\end{tabular}


==> tmp/figures/statistical_tests/BRATSMetric_2.tex <==
\begin{tabular}{p{0.167\textwidth}p{0.167\textwidth}p{0.167\textwidth}p{0.167\textwidth}p{0.167\textwidth}}
\hline
{} &     Class-wise \newline Variance &     One vs all \newline Entropy &           One vs all \newline MI \\
\hline
Class-wise \newline Entropy  &  $\textbf{[0.06, 0.16]}$ &  $\textbf{[0.0, 0.04]}$ &  $\textbf{[0.01, 0.06]}$ \\
Class-wise \newline Variance &                         &  $\textbf{[0.0, 0.03]}$ &  $\textbf{[0.01, 0.06]}$ \\
One vs all \newline Entropy  &                         &                        &   $\textbf{[0.96, 1.0]}$ \\
\hline
\end{tabular}


==> tmp/figures/vizualize.tex <==
% This file was created by tikzplotlib v0.9.4.
\begin{tikzpicture}

\begin{groupplot}[group style={group size=6 by 3}]
\nextgroupplot[
tick pos=left,
title={T1w
pre-contrast},
xmin=-0.5, xmax=127.5,
y dir=reverse,
ylabel={Dice = 0.784},
ymin=-0.5, ymax=127.5
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=127.5, ymin=127.5, ymax=-0.5] {vizualize-072.png};

\nextgroupplot[
tick pos=left,
title={Prediction},
xmin=-0.5, xmax=127.5,
y dir=reverse,
ymin=-0.5, ymax=127.5
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=127.5, ymin=127.5, ymax=-0.5] {vizualize-073.png};

\nextgroupplot[
tick pos=left,
title={Averaged
variance},
xmin=-0.5, xmax=127.5,
y dir=reverse,
ymin=-0.5, ymax=127.5
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=127.5, ymin=127.5, ymax=-0.5] {vizualize-074.png};

\nextgroupplot[
tick pos=left,
title={Averaged
entropy},
xmin=-0.5, xmax=127.5,
y dir=reverse,
ymin=-0.5, ymax=127.5
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=127.5, ymin=127.5, ymax=-0.5] {vizualize-075.png};

\nextgroupplot[
tick pos=left,
title={BC},
xmin=-0.5, xmax=127.5,
y dir=reverse,
ymin=-0.5, ymax=127.5
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=127.5, ymin=127.5, ymax=-0.5] {vizualize-076.png};

\nextgroupplot[
tick pos=left,
title={KL},
xmin=-0.5, xmax=127.5,
y dir=reverse,
ymin=-0.5, ymax=127.5
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=127.5, ymin=127.5, ymax=-0.5] {vizualize-077.png};

\nextgroupplot[
tick pos=left,
xmin=-0.5, xmax=127.5,
y dir=reverse,
ylabel={Dice = 0.861},
ymin=-0.5, ymax=127.5
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=127.5, ymin=127.5, ymax=-0.5] {vizualize-078.png};

\nextgroupplot[
tick pos=left,
xmin=-0.5, xmax=127.5,
y dir=reverse,
ymin=-0.5, ymax=127.5
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=127.5, ymin=127.5, ymax=-0.5] {vizualize-079.png};

\nextgroupplot[
tick pos=left,
xmin=-0.5, xmax=127.5,
y dir=reverse,
ymin=-0.5, ymax=127.5
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=127.5, ymin=127.5, ymax=-0.5] {vizualize-080.png};

\nextgroupplot[
tick pos=left,
xmin=-0.5, xmax=127.5,
y dir=reverse,
ymin=-0.5, ymax=127.5
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=127.5, ymin=127.5, ymax=-0.5] {vizualize-081.png};

\nextgroupplot[
tick pos=left,
xmin=-0.5, xmax=127.5,
y dir=reverse,
ymin=-0.5, ymax=127.5
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=127.5, ymin=127.5, ymax=-0.5] {vizualize-082.png};

\nextgroupplot[
tick pos=left,
xmin=-0.5, xmax=127.5,
y dir=reverse,
ymin=-0.5, ymax=127.5
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=127.5, ymin=127.5, ymax=-0.5] {vizualize-083.png};

\nextgroupplot[
tick pos=left,
xmin=-0.5, xmax=127.5,
y dir=reverse,
ylabel={Dice = 0.917},
ymin=-0.5, ymax=127.5
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=127.5, ymin=127.5, ymax=-0.5] {vizualize-084.png};

\nextgroupplot[
tick pos=left,
xmin=-0.5, xmax=127.5,
y dir=reverse,
ymin=-0.5, ymax=127.5
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=127.5, ymin=127.5, ymax=-0.5] {vizualize-085.png};

\nextgroupplot[
tick pos=left,
xmin=-0.5, xmax=127.5,
y dir=reverse,
ymin=-0.5, ymax=127.5
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=127.5, ymin=127.5, ymax=-0.5] {vizualize-086.png};

\nextgroupplot[
tick pos=left,
xmin=-0.5, xmax=127.5,
y dir=reverse,
ymin=-0.5, ymax=127.5
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=127.5, ymin=127.5, ymax=-0.5] {vizualize-087.png};

\nextgroupplot[
tick pos=left,
xmin=-0.5, xmax=127.5,
y dir=reverse,
ymin=-0.5, ymax=127.5
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=127.5, ymin=127.5, ymax=-0.5] {vizualize-088.png};

\nextgroupplot[
tick pos=left,
xmin=-0.5, xmax=127.5,
y dir=reverse,
ymin=-0.5, ymax=127.5
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=127.5, ymin=127.5, ymax=-0.5] {vizualize-089.png};
\end{groupplot}

\end{tikzpicture}


==> tmp/tables/AUCPRClassWiseMetric_0.tex <==
\begin{tabular}{p{0.167\textwidth}|p{0.167\textwidth}|p{0.167\textwidth}|p{0.167\textwidth}}
\hline
{} &     CW variance &      1vA Entropy &           1vA MI \\
\hline
CW Entropy  &  $\textbf{[0.31, 0.46]}$ &   $\textbf{[0.09, 0.20]}$ &          $[0.39, 0.55]$ \\
CW variance &                         &  $\textbf{[0.07, 0.17]}$ &   $\textbf{[0.90, 0.98]}$ \\
1vA Entropy  &                         &                         &  $\textbf{[0.87, 0.96]}$ \\
\hline
\end{tabular}


==> tmp/tables/AUCPRClassWiseMetric_1.tex <==
\begin{tabular}{p{0.167\textwidth}|p{0.167\textwidth}|p{0.167\textwidth}|p{0.167\textwidth}}
\hline
{} &     CW variance &      1vA Entropy &           1vA MI \\
\hline
CW Entropy  &  $\textbf{[0.26, 0.41]}$ &  $\textbf{[0.03, 0.11]}$ &          $[0.36, 0.52]$ \\
CW variance &                         &  $\textbf{[0.03, 0.11]}$ &  $\textbf{[0.94, 0.99]}$ \\
1vA Entropy  &                         &                         &  $\textbf{[0.92, 0.98]}$ \\
\hline
\end{tabular}


==> tmp/tables/AUCPRClassWiseMetric_2.tex <==
\begin{tabular}{p{0.167\textwidth}|p{0.167\textwidth}|p{0.167\textwidth}|p{0.167\textwidth}}
\hline
{} &     CW Variance &      1vA Entropy &          1vA MI \\
\hline
CW Entropy  &  $\textbf{[0.33, 0.48]}$ &  $\textbf{[0.06, 0.16]}$ &         $[0.45, 0.61]$ \\
CW Variance &                         &  $\textbf{[0.01, 0.06]}$ &  $\textbf{[0.95, 1.00]}$ \\
1vA Entropy  &                         &                         &  $\textbf{[0.95, 1.00]}$ \\
\hline
\end{tabular}


==> tmp/tables/AUCPRMetric.tex <==
\begin{tabular}{p{0.14\textwidth}|p{0.14\textwidth}|p{0.14\textwidth}|p{0.14\textwidth}|p{0.14\textwidth}|p{0.14\textwidth}}
\hline
& Av Variance &     Mu Entropy &          Mu MI &           Sim BC &           Sim KL \\
\hline
Av Entropy    &    $[0.43, 0.59]$ &   $\textbf{[0.20, 0.35]}$ &  $\textbf{[0.29, 0.45]}$ &  $\textbf{[0.89, 0.97]}$ &   $\textbf{[0.90, 0.98]}$ \\
Av Variance   &                   &  $\textbf{[0.22, 0.37]}$ &   $\textbf{[0.30, 0.46]}$ &  $\textbf{[0.93, 0.99]}$ &  $\textbf{[0.91, 0.98]}$ \\
Mu Entropy &                   &                         &          $[0.49, 0.65]$ &  $\textbf{[0.93, 0.99]}$ &   $\textbf{[0.95, 1.00]}$ \\
Mu MI      &                   &                         &                         &  $\textbf{[0.89, 0.97]}$ &  $\textbf{[0.91, 0.98]}$ \\
Sim BC       &                   &                         &                         &                         &  $\textbf{[0.64, 0.79]}$ \\
\hline
\end{tabular}


==> tmp/tables/AUCROCMetric.tex <==
\begin{tabular}{p{0.25\textwidth}p{0.25\textwidth}p{0.25\textwidth}}
\hline
{} &          Multi-class MI \\
\hline
Multi-class Entropy &  $\textbf{[0.29, 0.45]}$ \\
\hline
\end{tabular}


==> tmp/tables/BRATSMetric_0.tex <==
\begin{tabular}{p{0.167\textwidth}|p{0.167\textwidth}|p{0.167\textwidth}|p{0.167\textwidth}}
\hline
{} &     CW Variance &     1vA Entropy &          1vA MI \\
\hline
CW Entropy  &  $\textbf{[0.89, 0.97]}$ &  $\textbf{[0.96, 1.00]}$ &  $\textbf{[0.96, 1.00]}$ \\
CW Variance &                         &  $\textbf{[0.96, 1.00]}$ &  $\textbf{[0.97, 1.00]}$ \\
1vA Entropy  &                         &                        &  $\textbf{[0.00, 0.04]}$ \\
\hline
\end{tabular}


==> tmp/tables/BRATSMetric_1.tex <==
\begin{tabular}{p{0.167\textwidth}|p{0.167\textwidth}|p{0.167\textwidth}|p{0.167\textwidth}}
\hline
{} &    CW Variance &     1vA Entropy &           1vA MI \\
\hline
CW Entropy  &  $\textbf{[0.79, 0.90]}$ &  $\textbf{[0.95, 1.00]}$ &  $\textbf{[0.89, 0.97]}$ \\
CW Variance &                        &  $\textbf{[0.97, 1.00]}$ &   $\textbf{[0.96, 1.00]}$ \\
1vA Entropy  &                        &                        &   $\textbf{[0.00, 0.03]}$ \\
\hline
\end{tabular}


==> tmp/tables/BRATSMetric_2.tex <==
\begin{tabular}{p{0.167\textwidth}|p{0.167\textwidth}|p{0.167\textwidth}|p{0.167\textwidth}}
\hline
{} &     CW Variance &     1vA Entropy &           1vA MI \\
\hline
CW Entropy  &  $\textbf{[0.84, 0.94]}$ &  $\textbf{[0.96, 1.00]}$ &  $\textbf{[0.94, 0.99]}$ \\
CW Variance &                         &  $\textbf{[0.97, 1.00]}$ &  $\textbf{[0.94, 0.99]}$ \\
1vA Entropy  &                         &                        &   $\textbf{[0.00, 0.04]}$ \\
\hline
\end{tabular}


==> tmp/tables/ethnicity_table.tex <==
\begin{tabular}{c|c}
\hline
{} &  Ethnicity \\
\hline
Caucasian            &        141 \\
East Asia            &          2 \\
Afro-american        &          1 \\
South Asia and Hindu &          1 \\
\hline
\end{tabular}


==> tmp/tables/top_10_statistics/AUCPRClassWiseMetric_0.tex <==
\begin{tabular}{p{0.167\textwidth}|p{0.167\textwidth}|p{0.167\textwidth}|p{0.167\textwidth}p{0.167\textwidth}}
\hline
{} &    CW Variance &      1vA Entropy &           1vA MI \\
\hline
CW Entropy  &  $\textbf{[0.17, 0.40]}$ &  $\textbf{[0.07, 0.25]}$ &  $\textbf{[0.23, 0.48]}$ \\
CW Variance &                        &  $\textbf{[0.02, 0.16]}$ &  $\textbf{[0.84, 0.98]}$ \\
1vA Entropy  &                        &                         &  $\textbf{[0.84, 0.98]}$ \\
\hline
\end{tabular}


==> tmp/tables/top_10_statistics/AUCPRClassWiseMetric_1.tex <==
\begin{tabular}{p{0.167\textwidth}|p{0.167\textwidth}|p{0.167\textwidth}|p{0.167\textwidth}p{0.167\textwidth}}
\hline
{} &     CW Variance &      1vA Entropy &           1vA MI \\
\hline
CW Entropy  &  $\textbf{[0.18, 0.42]}$ &  $\textbf{[0.01, 0.13]}$ &  $\textbf{[0.22, 0.46]}$ \\
CW Variance &                         &    $\textbf{[0.00, 0.10]}$ &    $\textbf{[0.90, 1.00]}$ \\
1vA Entropy  &                         &                         &    $\textbf{[0.90, 1.00]}$ \\
\hline
\end{tabular}


==> tmp/tables/top_10_statistics/AUCPRClassWiseMetric_2.tex <==
\begin{tabular}{p{0.167\textwidth}|p{0.167\textwidth}|p{0.167\textwidth}|p{0.167\textwidth}p{0.167\textwidth}}
\hline
{} & CW Variance &      1vA Entropy &           1vA MI \\
\hline
CW Entropy  &      $[0.35, 0.61]$ &  $\textbf{[0.22, 0.46]}$ &           $[0.40, 0.67]$ \\
CW Variance &                     &  $\textbf{[0.02, 0.16]}$ &  $\textbf{[0.77, 0.95]}$ \\
1vA Entropy  &                     &                         &  $\textbf{[0.82, 0.97]}$ \\
\hline
\end{tabular}


==> tmp/tables/top_10_statistics/AUCPRMetric.tex <==
\begin{tabular}{p{0.14\textwidth}|p{0.14\textwidth}|p{0.14\textwidth}|p{0.14\textwidth}|p{0.14\textwidth}|p{0.14\textwidth}p{0.14\textwidth}}
\hline
{} &       AV Variance &     Mu Entropy &         Mu MI &          Sim BC &           Sim KL \\
\hline
AV Entropy    &  $\textbf{[0.23, 0.48]}$ &  $\textbf{[0.07, 0.25]}$ &  $\textbf{[0.09, 0.30]}$ &   $\textbf{[0.90, 1.00]}$ &    $\textbf{[0.90, 1.00]}$ \\
AV Variance   &                         &    $\textbf{[0.00, 0.10]}$ &         $[0.26, 0.52]$ &  $\textbf{[0.93, 1.00]}$ &   $\textbf{[0.93, 1.00]}$ \\
Mu Entropy &                         &                         &         $[0.42, 0.68]$ &  $\textbf{[0.93, 1.00]}$ &   $\textbf{[0.93, 1.00]}$ \\
Mu MI      &                         &                         &                        &  $\textbf{[0.93, 1.00]}$ &   $\textbf{[0.93, 1.00]}$ \\
Sim BC       &                         &                         &                        &                        &  $\textbf{[0.58, 0.82]}$ \\
\hline
\end{tabular}


==> tmp/tables/top_10_statistics/BRATSMetric_0.tex <==
\begin{tabular}{p{0.167\textwidth}|p{0.167\textwidth}|p{0.167\textwidth}|p{0.167\textwidth}p{0.167\textwidth}}
\hline
{} &    CW Variance &     1vA Entropy &          1vA MI \\
\hline
CW Entropy  &  $\textbf{[0.93, 1.00]}$ &  $\textbf{[0.93, 1.00]}$ &  $\textbf{[0.93, 1.00]}$ \\
CW Variance &                        &  $\textbf{[0.93, 1.00]}$ &  $\textbf{[0.93, 1.00]}$ \\
1vA Entropy  &                        &                        &  $\textbf{[0.00, 0.07]}$ \\
\hline
\end{tabular}


==> tmp/tables/top_10_statistics/BRATSMetric_1.tex <==
\begin{tabular}{p{0.167\textwidth}|p{0.167\textwidth}|p{0.167\textwidth}|p{0.167\textwidth}p{0.167\textwidth}}
\hline
{} &     CW Variance &     1vA Entropy &          1vA MI \\
\hline
CW Entropy  &  $\textbf{[0.82, 0.97]}$ &  $\textbf{[0.93, 1.00]}$ &  $\textbf{[0.93, 1.00]}$ \\
CW Variance &                         &  $\textbf{[0.93, 1.00]}$ &  $\textbf{[0.93, 1.00]}$ \\
1vA Entropy  &                         &                        &  $\textbf{[0.00, 0.07]}$ \\
\hline
\end{tabular}


==> tmp/tables/top_10_statistics/BRATSMetric_2.tex <==
\begin{tabular}{p{0.167\textwidth}|p{0.167\textwidth}|p{0.167\textwidth}|p{0.167\textwidth}p{0.167\textwidth}}
\hline
{} &   CW Variance &     1vA Entropy &          1vA MI \\
\hline
CW Entropy  &  $\textbf{[0.90, 1.00]}$ &  $\textbf{[0.93, 1.00]}$ &  $\textbf{[0.93, 1.00]}$ \\
CW Variance &                       &  $\textbf{[0.93, 1.00]}$ &  $\textbf{[0.93, 1.00]}$ \\
1vA Entropy  &                       &                        &  $\textbf{[0.00, 0.07]}$ \\
\hline
\end{tabular}

